Bring Your Own Instanton: Monopole Catalysis from Sourced SU(2) Instantons

We show that Rubakov-Callan catalysis of proton decay in the field of a 't Hooft-Polyakov monopole proceeds through "sourced SU(2) instantons", which are novel topological gauge configurations sourced by fermions and carrying unit instanton number. Unlike vacuum BPST instantons, these sourced instantons do not give rise to exponentially suppressed rates. We relate the winding number to the number of fermionic zero modes, suggesting an underlying index theorem for sourced instantons. We also calculate the closed-form expression for the leading-order correlator for fermion insertions both outside and inside the monopole core. Our results indicate that Rubakov-Callan catalysis is an IR effect where the scattering fermions do not reach the monopole core.

==> radial-diagrams.tex <==
% Load once in the preamble, before \begin{document}.
% Contains the drawing definitions used in Appendix A.3.
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta,decorations.pathmorphing,decorations.markings}

% Radial fermion propagator and local bosonic insertions.
\newcommand{\radialpropdiagram}{\vcenter{\hbox{%
	\colorlet{rulecolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=rulecolor,text=rulecolor,font=\small]
		\draw[line width=.6pt,-{Stealth[length=1.7mm,width=1.2mm]}] (-6,0)--(0,0);
		\draw[line width=.6pt] (0,0)--(6,0);
	\end{tikzpicture}%
}}}
\newcommand{\radialonevertex}[2]{\vcenter{\hbox{%
	\colorlet{rulecolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=rulecolor,text=rulecolor,font=\small,
		photon/.style={decorate,decoration={snake,amplitude=.7pt,segment length=3.8pt}}]
		\draw[line width=.6pt,-{Stealth[length=1.5mm,width=1mm]}] (-9,0)--(-2,0);
		\draw[line width=.6pt,-{Stealth[length=1.5mm,width=1mm]}] (0,0)--(8,0);
		\draw[line width=.6pt] (-2,0)--(0,0);
		\draw[line width=.6pt,#1] (0,0)--(0,7);
		\fill (0,0) circle (.6);
		\node[above,inner sep=1pt] at (0,7) {$#2$};
	\end{tikzpicture}%
}}}
\newcommand{\radialtwovertex}[2]{\vcenter{\hbox{%
	\colorlet{rulecolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=rulecolor,text=rulecolor,font=\small]
		\draw[line width=.6pt,-{Stealth[length=1.5mm,width=1mm]}] (-9,0)--(-2,0);
		\draw[line width=.6pt,-{Stealth[length=1.5mm,width=1mm]}] (0,0)--(8,0);
		\draw[line width=.6pt] (-2,0)--(0,0);
		\draw[line width=.6pt,dashed] (-5,7)--(0,0)--(5,7);
		\fill (0,0) circle (.6);
		\node[above,inner sep=1pt] at (-5,7) {$#1$};
		\node[above,inner sep=1pt] at (5,7) {$#2$};
	\end{tikzpicture}%
}}}


% One-loop diagrams with the same line styles as the vertex rules.
\newcommand{\radiallooptadpole}[1]{\vcenter{\hbox{%
	\colorlet{loopcolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=loopcolor,text=loopcolor,font=\small]
		\draw[line width=.6pt,postaction={decorate},decoration={markings,
			mark=at position .25 with {\arrow[rotate=-10]{Stealth[length=1.5mm,width=1mm]}}}]
			(0,0) circle (4);
		\draw[line width=.6pt,dashed] (4,0)--(11,0);
		\fill (4,0) circle (.6);
		\node[right,inner sep=1pt] at (11,0) {$#1$};
	\end{tikzpicture}%
}}}
\newcommand{\radialloopcontact}[2]{\vcenter{\hbox{%
	\colorlet{loopcolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=loopcolor,text=loopcolor,font=\small]
		\draw[line width=.6pt,postaction={decorate},decoration={markings,
			mark=at position .25 with {\arrow[rotate=-10]{Stealth[length=1.5mm,width=1mm]}}}]
			(0,0) circle (4);
		\draw[line width=.6pt,dashed] (11,3)--(4,0)--(11,-3);
		\fill (4,0) circle (.6);
		\node[right,inner sep=1pt] at (11,3) {$#1$};
		\node[right,inner sep=1pt] at (11,-3) {$#2$};
	\end{tikzpicture}%
}}}
\newcommand{\radialloopbubble}[2]{\vcenter{\hbox{%
	\colorlet{loopcolor}{.}%
	\begin{tikzpicture}[x=1mm,y=1mm,draw=loopcolor,text=loopcolor,font=\small]
		\draw[line width=.6pt,postaction={decorate},decoration={markings,
			mark=at position .25 with {\arrow[rotate=-10]{Stealth[length=1.5mm,width=1mm]}},
			mark=at position .75 with {\arrow[rotate=-10]{Stealth[length=1.5mm,width=1mm]}}}]
			(0,0) circle (4);
		\draw[line width=.6pt,dashed] (-10,0)--(-4,0);
		\draw[line width=.6pt,dashed] (4,0)--(10,0);
		\fill (-4,0) circle (.6);
		\fill (4,0) circle (.6);
		\node[left,inner sep=1pt] at (-10,0) {$#1$};
		\node[right,inner sep=1pt] at (10,0) {$#2$};
	\end{tikzpicture}%
}}}

